CRYLOGGER: Detecting Crypto Misuses Dynamically

Cryptographic (crypto) algorithms are the essential ingredients of all secure systems: crypto hash functions and encryption algorithms, for example, can guarantee properties such as integrity and confidentiality. Developers, however, can misuse the application programming interfaces (API) of such algorithms by using constant keys and weak passwords. This paper presents CRYLOGGER, the first open-source tool to detect crypto misuses dynamically. CRYLOGGER logs the parameters that are passed to the crypto APIs during the execution and checks their legitimacy offline by using a list of crypto rules. We compare CRYLOGGER with CryptoGuard, one of the most effective static tools to detect crypto misuses. We show that our tool complements the results of CryptoGuard, making the case for combining static and dynamic approaches. We analyze 1780 popular Android apps downloaded from the Google Play Store to show that CRYLOGGER can detect crypto misuses on thousands of apps dynamically and automatically. We reverse-engineer 28 Android apps and confirm the issues flagged by CRYLOGGER. We also disclose the most critical vulnerabilities to app developers and collect their feedback.

==> Makefile <==
# Makefile

# .tex file
PAPER = paper 

# .bib file
REFS = ref.bib

# tex compiler
LATEXCC = pdflatex

# Dependencies

# .tex files
TEX_DEPS = $(wildcard $(PAPER).tex) \
           $(wildcard tables/*.tex)

# Makefile rules

# main target
all: $(PAPER).pdf

# paper pdf generation
$(PAPER).pdf: $(TEX_DEPS) $(REFS)
	$(LATEXCC) $(PAPER)
	bibtex $(PAPER)	
	$(LATEXCC) $(PAPER)
	$(LATEXCC) $(PAPER)

# clean the generated file
clean:
	rm -f *.aux *.blg *.log *.out $(PAPER).pdf

.PHONY: all clean gnu


==> tables/times.tex <==

\begin{table}
\caption{\normalfont Comparison on average running time on 150 Android apps.}\label{table:times}
\centering
\begin{tabular}{cccc}
\toprule
\textbf{\lowercase \our{10}} &
\textbf{\lowercase \our{30}} &
\textbf{\lowercase \our{50}} &
\textbf{\lowercase \cryptoguardname} \\
\midrule
xx & 287.4 sec & xx & 287.6 sec \\
\bottomrule
\end{tabular}
\end{table}

